AIREX: Neural Network-based Approach for Air Quality Inference in Unmonitored Cities

Urban air pollution is a major environmental problem affecting human health and quality of life. Monitoring stations have been established to continuously obtain air quality information, but they do not cover all areas. Thus, there are numerous methods for spatially fine-grained air quality inference. Since existing methods aim to infer air quality of locations only in monitored cities, they do not assume inferring air quality in unmonitored cities. In this paper, we first study the air quality inference in unmonitored cities. To accurately infer air quality in unmonitored cities, we propose a neural network-based approach AIREX. The novelty of AIREX is employing a mixture-of-experts approach, which is a machine learning technique based on the divide-and-conquer principle, to learn correlations of air quality between multiple cities. To further boost the performance, it employs attention mechanisms to compute impacts of air quality inference from the monitored cities to the locations in the unmonitored city. We show, through experiments on a real-world air quality dataset, that AIREX achieves higher accuracy than state-of-the-art methods.

==> algorithms/traning_method.tex <==

\begin{algorithm}[!t]
\caption{\textsc{Training} \label{alg:training}}
	{\small
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	            \SetKwInOut{Hyper}{HyperParameter}
	            \SetKwFunction{Expand}{Expand}
\Input{$\{\textit{\textbf{A}}_{1},\textit{\textbf{P}}_{1},\textit{\textbf{R}}_{1},\textit{\textbf{M}}_{1},\ldots,\textit{\textbf{A}}_{|\textit{\textbf{C}}|},\textit{\textbf{P}}_{|\textit{\textbf{C}}|},\textit{\textbf{R}}_{|\textit{\textbf{C}}|},\textit{\textbf{M}}_{|\textit{\textbf{C}}|}\}$, $\{\textit{\textbf{P}}_{\tilde{c}},\textit{\textbf{R}}_{\tilde{c}},\textit{\textbf{M}}_{\tilde{c}}\}$}
\Hyper{$\lambda$, $\gamma$, $\zeta$}
set $\cup_{\tilde{s} \in \tilde{\textit{\textbf{S}}}} \{\mathbb{X}_{\tilde{s}}^{local}\}$ from $\{\textit{\textbf{P}}_{\tilde{c}},\textit{\textbf{R}}_{\tilde{c}},\textit{\textbf{M}}_{\tilde{c}}\}$\\
$\textbf{Repeat}$\\
     \ForEach{$c_{m} \in \sourcecities$}{
        set $\{\textit{\textbf{A}}_{m},\textit{\textbf{P}}_{m},\textit{\textbf{R}}_{m}\}$ in the city $c_{m}$ as a meta-target;\\
        set $\cup_{c_{m'}\neq c_{m}}{\{\textit{\textbf{A}}_{m'},\textit{\textbf{P}}_{m'},\textit{\textbf{R}}_{m'}\}}$ as meta-sources;\\
        select $\featuretarget$ randomly from $\featurestation$ in the meta-target;\\
        set $\cup_{c_{m'}\neq c_{m}} \{\cup_{s_{i} \in \textit{\textbf{S}}_{m'}} \{\mathbb{X}_{s_{i}}^{station}\}\}$ from all the meta-sources\\
        set $\cup_{c_{m'}\neq c_{m}} \{\mathbb{X}_{c_{m'}}^{city}\}$ from all the meta-sources
        
         \ForEach{$\textit{\textbf{{X}}}^{local}$, $\cup_{c_{m'}\neq c_{m}} \{\cup_{s_{i} \in \textit{\textbf{S}}_{m'}} \{\textit{\textbf{{X}}}_{s_{i}}^{station}\}\}$, $\cup_{c_{m'}\neq c_{m}} \{\textit{\textbf{{X}}}_{c_{m'}}^{city}\}$, $\cup_{\tilde{s} \in \tilde{\textit{\textbf{S}}}} \{\textit{\textbf{{X}}}_{\tilde{s}}^{local}\}$, $y$}{
              $\textbf{z}_{\tilde{l}}^{(L+L'')}$ $\gets$ Encode($\textit{\textbf{{X}}}^{local}$)\\
             \ForEach{$c_{k}$}{
                  $\{\textbf{z}_{k1}^{(L+L'')},\ldots,\textbf{z}_{kn}^{(L+L'')}\}$ $\gets$ Encode($\cup_{s_{i} \in \textit{\textbf{S}}_{k}} \{\textit{\textbf{{X}}}_{s_{i}}^{station}\}$)
                  $\textbf{z}_{k}$ $\gets$ SA($\{\textbf{z}_{k1}^{(L+L'')},\ldots,\textbf{z}_{kn}^{(L+L'')}\}$)
                  $\tilde{y}_{c_{k}}$ $\gets$ Mid-Output($\textbf{z}_{\tilde{l}}^{(L+L'')}$, $\textbf{z}_{k}$)
             }
               $\{\beta_{c1},\ldots,\beta_{c_{k}}\}$ $\gets$ CA($\{\textbf{z}_{\tilde{l}}^{(L+L'')}$, $\textbf{z}_{k1}^{(L+L'')},\ldots,\textbf{z}_{kn}^{(L+L'')}\}$, $\textit{\textbf{{X}}}_{c_{k}}^{city}$)\\
              $\tilde{y}$ $\gets$ Output($\{\beta_{c1},\ldots,\beta_{c_{k}}\}$, $\{\tilde{y}_{c1},\ldots,\tilde{y}_{c_{k}}\}$)\\
               Compute $\mathcal{L}_{pred}$($\tilde{y}$, $y$)\\
               Compute $\mathcal{L}_{mean}$($\{\tilde{y}_{c1},\ldots,\tilde{y}_{c_{k}}\}$, $y$)\\
               set $\cup_{c_{m'}\neq c_{m}}$ \{$\cup_{s_{i} \in \textit{\textbf{S}}_{m'}}$\\ $\{\textit{\textbf{{X}}}_{s_{i}}^{local}\}$\} from $\cup_{c_{m'}\neq c_{m}}$ \{$\cup_{s_{i} \in \textit{\textbf{S}}_{m'}} \{\textit{\textbf{{X}}}_{s_{i}}^{station}\}\}$\\
            %   Compute $\mathcal{L}_{adv}$($\cup_{c_{m'}\neq c_{m}}$ \{Encode($\cup_{s_{i} \in \textit{\textbf{S}}_{m'}}\\ \{\textit{\textbf{{X}}}_{s_{i}}^{local}\}$)\}, Encode($\cup_{\tilde{s} \in \tilde{\textit{\textbf{S}}}} \{\textit{\textbf{{X}}}_{\tilde{s}}^{local}\}$))
            %   Compute $\mathcal{R}$($\{\beta_{c1},\ldots,\beta_{c_{k}}\}$)\\
            %   Compute $\mathcal{L}=\lambda\cdot\mathcal{L}_{pred}+(1-\lambda)\cdot\mathcal{L}_{mean}+\gamma\cdot\mathcal{L}_{adv}+\eta\cdot\mathcal{R}$\\
            %   Update parameters via back-propagating gradients of the $\mathcal{L}$\\
        }
    }
$\textbf{Until}$ converging the total loss $\mathcal{L}$
}
\end{algorithm}

==> result_entropy.tex <==

% \begin{figure*}[!h]
%     \centering
%     \includegraphics[keepaspectratio, scale=0.5, angle=0]
%                     {figure/legend.pdf}
%     %\caption{Caption}
%     \label{fig:my_label}
% \end{figure*}
%\vspace{-10mm}

\begin{figure*}[!h]
  \centering
    \begin{tabular}{c}

       \begin{minipage}{1.0\hsize}
        \centering
    \includegraphics[keepaspectratio, scale=0.4, angle=0]
                    {figure/legend.pdf}
      \end{minipage}%\vspace{-1mm}
 \\
%----- y = sin(x) -----
 
      \begin{minipage}{0.245\hsize}
        \centering
          \includegraphics[keepaspectratio, scale=0.225, angle=0]{figure/cora_ent_metrics.pdf}
                    %{figure/cora_ent_metrics.pdf}
                    
                          \caption*{(a) Cora}
                          \label{cora_ent}
      \end{minipage}
 
%--- 中央スペース
 
    %   \begin{minipage}{0.02\hsize}
    %     \vspace{-10mm}
    %   \end{minipage}
 
%----- y = sin(2x) -----
 
      \begin{minipage}{0.245\hsize}
        \centering
          \includegraphics[keepaspectratio, scale=0.225, angle=0]{figure/cite_ent_metrics.pdf}
                          %{figure/cite_ent_metrics.pdf}
                          
                          \caption*{(b) Citeseer}
                          \label{cite_ent}
      \end{minipage} %\\
 
%--- 上下スペース
 
    %   \begin{minipage}{0.06\hsize}
    %     \vspace{-4mm}
    %   \end{minipage} \\
 
 
%----- y = sin(3x) -----
 
      \begin{minipage}{0.245\hsize}
        \centering
          \includegraphics[keepaspectratio, scale=0.225, angle=0]{figure/pubmed_ent_metrics.pdf}
          %{figure/pubmed_ent_metrics.pdf}
          
                          \caption*{(c) Pubmed}
                          \label{pubmed_ent}
      \end{minipage}
 
%--- 中央スペース
 
    %   \begin{minipage}{0.06\hsize}
    %     \hspace{5mm}
    %   \end{minipage}
 
 
%----- y = sin(4x) -----
 
      \begin{minipage}{0.245\hsize}
        \centering
          \includegraphics[keepaspectratio, scale=0.225, angle=0]{figure/wiki_ent_metrics.pdf}
                          %{figure/wiki_ent_metrics.pdf}
                          
                          \caption*{(d) Wiki}
                          \label{wiki_ent}
      \end{minipage}
 
 
    \end{tabular}
   \caption{Entropy and three metrics (ACC, NMI, F1) for clustering results: the metrics are expressed in percent.}
    \label{beta_plot}
\end{figure*}   


% \begin{figure*}
%     \centering
%     \includegraphics[keepaspectratio, scale=0.19, angle=0]
%                           {figure/beta_plot.pdf}
%     \caption{Entropy and clustering results: The plots are the results of Cora, Citesseer, Wiki, and Pubmed from left.}
%     \label{beta_plot}
% \end{figure*}

==> result_table.tex <==

% %%%%%%%%%%%%  cora  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[ht]
% \centering
% \begin{tabular}{llccc}  
% \toprule
% Methods  & Input & ACC (\%)  & NMI (\%) & F1 (\%) \\
% \midrule

% spectral & St  &  33.78  &  18.88  &  30.02 \\

% DANMF & St  &  53.22  &  39.18  &  38.62 \\ 

% DeepWalk & St  &  45.42  &  32.21 &  37.89 \\ \hline

% k-means & At  &  32.63  &  17.13  &  24.72 \\

% NMF & At  &  38.04  &  14.78  &  34.58 \\ \hline

% TADW & Both  &  52.74  &  35.87  &  40.15 \\

% %CDE & Both  &  0.0  &  0.0  &  0.0 \\

% GAE & Both  &  53.51  &  40.22  &  40.95 \\
% VGAE & Both  &  54.89  &  38.73  &  42.10 \\
% MGAE & Both  &  64.73  &  44.76  &  39.43 \\

% ARGE & Both  &  64.01  &  44.89  &  61.01 \\
% ARVGE & Both  &  63.80  &  45.55  & {\bf 62.61} \\
% \hline


% %BEST & Both  &  64.73  &  45.55  &  {\bf 62.61} \\


% GCNMF & Both  &  {\bf 66.29}  &  {\bf 50.74}  &  60.88 \\


% \bottomrule
% \end{tabular}
% \caption{Experimental results on Cora}
% \label{ex_results_cora}
% \end{table}



% %%%%%%%%% citeseer %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[ht]
% \centering
% \begin{tabular}{llccc}  
% \toprule
% Methods  & Input & ACC (\%)  & NMI (\%) & F1 (\%) \\
% \midrule

% spectral & St  &  24.89  &  12.54  &  28.99 \\

% DANMF & St  &  40.32  &  16.71  &  30.12 \\ 

% DeepWalk & St  &  31.75  &  8.97  &  25.78 \\ \hline

% k-means & At  &  39.32  &  18.07  &  31.57 \\

% NMF & At  &  46.89  &  20.35  &  43.43 \\ \hline

% TADW & Both  &  53.56  &  31.55  &  44.12 \\

% %CDE & Both  &  0.0  &  0.0  &  0.0 \\

% GAE & Both  &  42.27  &  19.11  &  30.44 \\
% VGAE & Both  &  46.11  &  23.46  &  32.98 \\

% MGAE & Both  &  63.79  &  39.88  &  41.31 \\

% ARGE & Both  &  58.10  &  35.11  &  55.89 \\
% ARVGE & Both  &  55.35  &  27.10  &  53.02 \\ \hline


% %BEST & Both  &  63.79  &  39.88 &  55.89 \\

%  GCNMF  & Both  &  {\bf 66.64}  &  {\bf 40.52}  &  {\bf 62.84} \\

% \bottomrule
% \end{tabular}
% \caption{Experimental results on Citeseer}
% \label{ex_results_cite}
% \end{table}


% %%%%%%%%%%%%  wiki  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[ht]
% \centering
% \begin{tabular}{llccc}  
% \toprule
% Methods  & Input & ACC (\%)  & NMI (\%) & F1 (\%) \\
% \midrule

% spectral & St  &  22.66  &  20.02  &  16.88 \\

% DANMF & St  &  40.33  &  33.11  &  34.45 \\ 

% DeepWalk & St  &  37.12  &  31.37  &  24.99 \\ \hline

% k-means & At  &  32.43  &  31.23  &  23.88 \\

% NMF & At  &  46.15  &  42.51  &  34.00 \\ \hline

% TADW & Both  &  31.67  &  28.22  &  21.45 \\

% %CDE & Both  &  0.0  &  0.0  &  0.0 \\

% GAE & Both  &  18.56  &  12.12  &  16.64 \\
% VGAE & Both  &  29.11  &  31.54  &  21.44 \\

% MGAE & Both  &  51.55  &  48.99  &  41.24 \\

% ARGE & Both  &  42.32  &  39.61  &  39.09 \\ 
% ARVGE & Both  &  41.75  &  41.21  &  38.22 \\  \hline


% %BEST & Both  &  51.55  &  48.99  &  41.24 \\


% GCNMF & Both  &  {\bf 55.76}  &  {\bf 54.95}  &  {\bf 46.45} \\
% \bottomrule
% \end{tabular}
% \caption{Experimental results on Wiki}
% \label{ex_results_wiki}
% \end{table}


% %%%%%%%%%%  pubmed  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[ht]
% \centering
% \begin{tabular}{llccc}  
% \toprule
% Methods  & Input & ACC (\%)  & NMI (\%) & F1 (\%) \\
% \midrule

% spectral & St  &  40.14  &  4.12  &  52.42 \\

% DANMF & St  &  61.27  &  21.18  &  46.56 \\ 

% DeepWalk & St  &  60.12  &  15.83  &  45.16 \\ \hline

% k-means & At  &  55.10  &  27.87  &  55.92 \\

% NMF & At  &  60.29  &  30.76  &  59.73 \\ \hline

% TADW & Both  &  57.12  &  23.11  &  49.65 \\

% %CDE & Both  &  0.0  &  0.0  &  0.0 \\

% GAE & Both  &  63.13  &  23.92  &  50.26 \\
% VGAE & Both  &  62.48  &  21.09  &  47.95 \\

% MGAE & Both  &  44.17  &  9.10  &  42.04 \\

% ARGE & Both  &  60.02  &  22.89  &  58.12 \\
% ARVGE & Both  &  59.08  &  21.52  &  23.56 \\ \hline


% %BEST & Both  &  63.13  &  30.76  &  59.73 \\


% GCNMF & Both  &  {\bf 63.41}  &  {\bf 32.81}  &  {\bf 63.34} \\

% \bottomrule
% \end{tabular}
% \caption{Experimental results on Pubmed}
% \label{ex_results_pubmed}
% \end{table}





\begin{table*}[ht]
    \centering
    
    \begin{tabular}{ll|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Input} &\multicolumn{3}{c|}{Cora} & \multicolumn{3}{c|}{Citeseer} & \multicolumn{3}{c|}{Pubmed} &\multicolumn{3}{c}{Wiki}\\ 

& & ACC & NMI & F1 & ACC & NMI & F1 & ACC & NMI & F1 & ACC & NMI & F1\\ \hline
spectral & S  &  33.78  &  18.88  &  30.02  &  24.89  &  12.54  &  28.99   &  40.14  &  4.12  &  52.42  &  22.66  &  20.02  &  16.88 \\
			
DANMF & S  &  53.22  &  39.18  &  38.62 &  40.32  &  16.71  &  30.12  &  61.27  &  21.18  &  46.56  &  40.33  &  33.11  &  34.45 \\
			
DeepWalk & S  &  45.42  &  32.21 &  37.89   &  31.75  &  8.97  &  25.78 &  60.12  &  15.83  &  45.16   &  37.12  &  31.37  &  24.99 \\ \hline
			
k-means & A  &  32.63  &  17.13  &  24.72   &  39.32  &  18.07  &  31.57  &  55.10  &  27.87  &  55.92  &  32.43  &  31.23  &  23.88 \\
			
NMF & A  &  38.04  &  14.78  &  34.58 &  46.89  &  20.35  &  43.43   &  60.29  &  30.76  &  59.73   &  46.15  &  42.51  &  34.00 \\ \hline
			
TADW & S+A  &  52.74  &  35.87  &  40.15   &  53.56  &  31.55  &  44.12  &  57.12  &  23.11  &  49.65  &  31.67  &  28.22  &  21.45 \\
			
GAE & S+A  &  53.51  &  40.22  &  40.95   &  42.27  &  19.11  &  30.44   &  63.13  &  23.92  &  50.26   &  18.56  &  12.12  &  16.64 \\
VGAE & S+A &  54.89  &  38.73  &  42.10  &  46.11  &  23.46  &  32.98   &  62.48  &  21.09  &  47.95   &  29.11  &  31.54  &  21.44 \\
MGAE & S+A  &  64.73  &  44.76  &  39.43   &  63.79  &  39.88  &  41.31   &  44.17  &  9.10  &  42.04   &  51.55  &  48.99  &  41.24 \\
ARGE & S+A  &  64.01  &  44.89  &  61.01  &  58.10  &  35.11  &  55.89   &  60.02  &  22.89  &  58.12   &  42.32  &  39.61  &  39.09 \\			
ARVGE & S+A  &  63.80  &  45.55  & {\bf 62.61}   &  55.35  &  27.10  &  53.02  &  59.08  &  21.52  &  23.56 &  41.75  &  41.21  &  38.22 \\  \hline
			
GCNMF & S+A  &  {\bf 66.29}  &  {\bf 50.74}  &  60.88  &  {\bf 66.64}  &  {\bf 40.52}  &  {\bf 62.84} &  {\bf 63.41}  &  {\bf 32.81}  &  {\bf 63.34} & {\bf 55.76}  &  {\bf 54.95}  &  {\bf 46.45} \\ \hline
\end{tabular}
    \caption{Experimental results on clustering: the metrics are expressed in percent.}
    \label{ex_result}
\end{table*}


==> result_visualization.tex <==
\begin{figure*}[ht]

\begin{tabular}{c}

\begin{minipage}{0.16\hsize}
  \begin{center}
   \includegraphics[keepaspectratio, scale=0.12, angle=0]{figure/raw_aa.pdf}\\
  \text{(a) Original attributes}
  \end{center}
  \end{minipage}
 
    \begin{minipage}{0.16\hsize}
    \begin{center}
    \includegraphics[keepaspectratio, scale=0.12, angle=0]{figure/beta10_aa.pdf}\\
    \text{(b) $\beta=10$}
    \end{center}
  
  \end{minipage}
  \begin{minipage}{0.16\hsize}
    \begin{center}
    \includegraphics[keepaspectratio, scale=0.12, angle=0]{figure/beta5_aa.pdf}\\
    \text{(c) $\beta=5$}
    \end{center}
  
  \end{minipage}
  
  \begin{minipage}{0.16\hsize}
    \begin{center}
    \includegraphics[keepaspectratio, scale=0.12, angle=0]{figure/beta1_aa.pdf}\\
    \text{(d) $\beta=1$}
    \end{center}
  
  \end{minipage}
 \begin{minipage}{0.16\hsize}
  \begin{center}
   \includegraphics[keepaspectratio, scale=0.12, angle=0]{figure/cora_FN.pdf}\\
  \text{(e) NMF with FN}
  \end{center}
  \end{minipage}
  \begin{minipage}{0.16\hsize}
  \begin{center}
   \includegraphics[keepaspectratio, scale=0.12, angle=0]{figure/NMF_aa.pdf}\\
  \text{(f) NMF with KL}
  \end{center}
  \end{minipage}
 
 
 \end{tabular}
 
 \caption{Two dimensional visualization of features in each step of GCNMF on Cora.}
 \label{vis_emb}
\end{figure*}
